Fine-Grained Erasure in Text-to-Image Diffusion-based Foundation Models

Existing unlearning algorithms in text-to-image generative models often fail to preserve the knowledge of semantically related concepts when removing specific target concepts: a challenge known as adjacency. To address this, we propose FADE (Fine grained Attenuation for Diffusion Erasure), introducing adjacency aware unlearning in diffusion models. FADE comprises two components: (1) the Concept Neighborhood, which identifies an adjacency set of related concepts, and (2) Mesh Modules, employing a structured combination of Expungement, Adjacency, and Guidance loss components. These enable precise erasure of target concepts while preserving fidelity across related and unrelated concepts. Evaluated on datasets like Stanford Dogs, Oxford Flowers, CUB, I2P, Imagenette, and ImageNet1k, FADE effectively removes target concepts with minimal impact on correlated concepts, achieving atleast a 12% improvement in retention performance over state-of-the-art methods.

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/X_suppl_bkp.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary


\section{Theoretical Basis for Concept Lattice}
\label{sec:rationale}
Based on the literature, as noted in the work from Duda et al. \cite{duda2001pattern}, we extend the observations of Boiman et al. \cite{boiman2008defense} as a theoretical justification for the proposed nearest neighbor-based concept lattice, which approximates the gold-standard Naive Bayes classifier for constructing the adjacency set. \\


\noindent\textbf{Theorem: k-Nearest Neighbor in $\mathbb{R}^d$ as an approximation to Naive Bayes.}


\noindent Let  $\mathbf{x} \in \mathbb{R}^{h \times w \times c}$  be an image, with  height, width, and number of channels as $h$,  $w$, and $c$, respectively. Let  $\phi: \mathbb{R}^{h \times w \times c} \to \mathbb{R}^d$  be the mapping function of $\mathbf{x}$ to a latent feature space $\mathbb{R}^d$, where  $d \ll hwc$. Assume that the latent features  $z := \phi(\mathbf{x})$  are conditionally independent given the class label  $C \in \mathcal{C}$. As the sample size  $N \to \infty$  and the number of neighbors  $k \to \infty$  with  $k/N \to 0$, the k-Nearest Neighbors (k-NN) classifier operating in $\mathbb{R}^d$ converges to the Bayes optimal classifier, which, under the conditional independence assumption, is the Naive Bayes classifier. Formally,


\begin{equation*}
\lim_{N \to \infty} P(C_{\text{K-NN}}(\phi(\mathbf{x})) = C_{\text{NB}}(\mathbf{x})) = 1.    
\end{equation*}


% \\ \noindent\textbf{Preliminaries and Notations}

\noindent\textbf{Proof Outline:}
\noindent Let  $D = \{(\mathbf{x}_i, y_i)\}_{i=1}^N$  be a dataset consisting of images  $\mathbf{x}_i \in \mathbb{R}^{h \times w \times c}$  and their corresponding class labels  $y_i \in \mathcal{C}$. Each image  $\mathbf{x}_i$  is mapped to a latent space  $\mathbb{R}^d$  through the mapping function  $\phi: \mathbb{R}^{h \times w \times c} \to \mathbb{R}^d$, resulting in a latent feature vector  $z_i := \phi(\mathbf{x}_i)$.

\noindent We assume the following:
\begin{itemize}
    \item The latent feature vectors  $\phi(\mathbf{x})$  are conditionally independent given the class label  $y$.
    \item The representation function $\phi(\mathbf{x})$  preserves the class-conditional structure in $\mathbb{R}^d$, such that images of the same class remain clustered in proximity to one another.
    \item $d$  is sufficiently large to ensure that $\mathbf{z}$ provides high separability between classes while remaining lower-dimensional than the original input space, i.e., in $d \ll hwc$.
\end{itemize} 


\noindent\textbf{Proof:} We follow the outline above proceeding step by step.

\noindent\textbf{Step 1: Bayes Optimal Classifier (Naive Bayes)}
\noindent The Bayes optimal classifier is defined as the classifier that minimizes the expected classification error by choosing the class that maximizes the posterior probability  $P(C = c | \mathbf{x})$. Under the Naive Bayes assumption, the posterior decomposes as follows:

\begin{equation}
    P(C = c | \mathbf{x}) = \frac{P(\mathbf{x} | C = c) P(C = c)}{P(\mathbf{x})}.    
\end{equation}


Given the conditional independence of $\mathbf{z}$ in $\mathbb{R}^d$, the class-conditional likelihood  $P(\mathbf{x} | C = c)$  is factorized over the components of the latent vector  $\phi(\mathbf{x}) = (\phi_1(\mathbf{x}), \ldots, \phi_d(\mathbf{x}))$ , i.e.,

\begin{equation}
    P(\mathbf{x} | C = c) = \prod_{j=1}^d P(\phi_j(\mathbf{x}) | C = c).
\end{equation}


Thus, the decision rule of the Naive Bayes classifier becomes:

\begin{equation}
    C_{\text{NB}}(\mathbf{x}) = \arg\max_{c \in \mathcal{C}} P(C = c) \prod_{j=1}^d P(\phi_j(\mathbf{x}) | C = c).
\end{equation}



\noindent\textbf{Step 2: k-Nearest Neighbor Classifier in $\mathbb{R}^d$}

\noindent The k-NN classifier operates in the latent space $\mathbb{R}^d$, assigns a class label $C_{\text{k-NN}}$ to a query vector $\phi(\mathbf{x})$ by selecting the nearest instance in $\mathbb{R}^d$. For two images $\mathbf{x}$  and  $\mathbf{x}_i$, we can defined it formally as:

\begin{equation}
    C_{\text{k-NN}} = \arg\max_{i} \text{sim}(\phi(\mathbf{x}), \phi(\mathbf{x}_i)) = \frac{\langle \phi(\mathbf{x}), \phi(\mathbf{x}_i) \rangle}{\|\phi(\mathbf{x})\| \|\phi(\mathbf{x}_i)\|}.
\end{equation}
    

The k-NN classifier assigns the label to the query image $\mathbf{x}$  by aggregating the labels of its k -nearest neighbors  $\mathcal{N}_k(\mathbf{x})$ in the latent space. This is formally described as:

\begin{equation}
    C_{\text{k-NN}}(\phi(\mathbf{x})) = \arg\max_{c \in \mathcal{C}} \sum_{\mathbf{x}_i \in \mathcal{N}_k(\mathbf{x})} \mathbb{I}(y_i = c),
\end{equation}


where  $\mathbb{I}(y_i = c)$  is the indicator function, returning 1 if  $y_i = c$  and $0$ otherwise. \\


\noindent\textbf{Step 3: Convergence of k-NN to Bayes Optimal Classifier}\\
\noindent As established by Covert \& Hart et al. \cite{cover1967nearest} in statistical learning theory, the k-NN classifier converges to the Bayes optimal classifier as $N \to \infty$, provided that $k \to \infty$  and  $k/N \to 0$. That is, for sufficiently large $N$ and $k$, the decision rule of the k-NN classifier approximates that of the Bayes optimal classifier $C_{\text{Bayes}(\mathbf{x})}$, i.e.,

\begin{equation}
\lim_{N \to \infty} P(C_{\text{K-NN}}(\phi(\mathbf{x})) = C_{\text{Bayes}}(\mathbf{x})) = 1.
\end{equation}

This convergence holds because, with increase in $N$, $\mathcal{N}_k(\mathbf{x})$ increasingly reflects the local distribution of data around $\mathbf{x}$, which aligns with the underlying class-conditional probability distribution. \\


\noindent\textbf{Step 4: Consistency of k-NN with Naive Bayes in $\mathbb{R}^d$}

\noindent Given the Naive Bayes assumption that the components  $\phi_j(\mathbf{x})$  of the latent representation  $\phi(\mathbf{x})$  are conditionally independent given the class label, the Bayes optimal classifier in this latent space is precisely the Naive Bayes classifier  $C_{\text{NB}}(\mathbf{x})$ . Therefore, we have:

\begin{equation}
    C_{\text{Bayes}}(\mathbf{x}) = C_{\text{NB}}(\mathbf{x}),
\end{equation}


where $C_{\text{Bayes}}(\mathbf{.})$ operates on the latent representations  $\phi(\mathbf{x})$. Combining equation 7 with the equation 6, we conclude that:

\begin{equation}
    \lim_{N \to \infty} P(C_{\text{K-NN}}(\phi(\mathbf{x})) = C_{\text{NB}}(\mathbf{x})) = 1.
\end{equation}



This establishes that the CLIP-based K-NN classifier converges to the Naive Bayes classifier as the sample size grows, provided the assumptions of conditional independence hold in the latent space $\mathbb{R}^d$.



\noindent\textbf{Remarks:}
\begin{itemize}
    \item In high-dimensional spaces, Bayers et al. \cite{beyer1999nearest} proposed concentration of distances implying that Euclidean distance and Cosine similarity perform similarly as $d \to \infty$, ensuring that the use of cosine similarity in latent space provides robust distance-based classification.
    \item In our implementation, the mapping function $\phi: \mathbb{R}^{h \times w \times c} \to \mathbb{R}^d$ is a pre-trained CLIP model, serving for dimensionality reduction where $d \ll hwc$.
    \item The CLIP model's latent space captures abstract and semantic features, reducing the dependency between the components of $\phi(\mathbf{x})$. This makes the assumption of conditional independence more plausible in $\mathbb{R}^d$, allowing Naive Bayes to model the class-conditional likelihoods accurately in the latent space.
    \item For k-NN to converge to optimal Bayes classifier, k must satisfy $k \to \infty$ and $N \to \infty$.    
\end{itemize}


\begin{figure}[]
%\vspace{-15pt}
\centering
  \includegraphics[scale=0.62]{Images/IA.pdf}
\caption{\textbf{Radar plot comparing FADE with existing unlearning methods (ESD, FMN, SPM, Receler).} For a fair analysis, methods with $A_{\text{er}} \leq 20\%$ are considered. The plot shows structural similarity scores (circular axis, \%) and adjacency accuracy (radial axes) on concepts from the ImageNet-1k dataset. Most methods begin to degrade beyond a similarity score of 70\%, with SPM remaining resilient until 90\% and FADE demonstrating the highest robustness.} 
    \label{fig:IA}
\end{figure}


\section{Adjacency Inflection Analysis}
This section examines the breaking point of existing algorithms in preserving adjacency—specifically, at what similarity threshold these methods begin to fail. To evaluate robustness, we analyze the performance of each algorithm as semantic similarity increases, using fine-grained classes from ImageNet-1k and other fine-grained datasets. Figure \ref{fig:IA} illustrates the relationship between CLIP-based semantic similarity (circular axis, %) and average adjacency accuracy (radial axes).

Results show that FMN and ESD degrade significantly at 78\% similarity, while Receler fails at 80\%. Although SPM demonstrates moderate resilience, it begins to falter beyond 90\% similarity, marking a critical threshold where all existing methods fail to preserve adjacency effectively. In stark contrast, FADE maintains high adjacency accuracy even at elevated similarity levels, demonstrating superior robustness. These findings validate FADE’s efficacy in adjacency-aware unlearning, outperforming state-of-the-art approaches under challenging fine-grained conditions.

% \footnotetext{For a fair analysis, methods with $A_{\text{er}} \leq 20\%$ are considered.}



\section{Extended Quantitative Results}
As previously discussed, we utilize Stanford Dogs, Oxford Flower, and CUB datasets to evaluate the proposed FADE and existing state-of-the-art algorithms. We present the adjacency set with their similarity scores in Table \ref{tab:similarity_scores}.

We report the classification accuracy for each class in the adjacency set of each target class from the Stanford Dogs, Oxford Flowers, and CUB datasets in Tables \ref{tab:adj_acc_stanford_dogs}, \ref{tab:adj_acc_oxford_flowers}, and \ref{tab:adj_acc_cub}. These results extend the findings reported in Table 1 of the main paper. The original model (SD) has not undergone any unlearning, so higher accuracy is better. The remaining models are comparison algorithms, and for each of them, the model should achieve lower accuracy on the target class to demonstrate better unlearning and higher accuracy on neighboring classes to show better retention of adjacent classes. From Tables \ref{tab:adj_acc_stanford_dogs}, \ref{tab:adj_acc_oxford_flowers}, and \ref{tab:adj_acc_cub}, it is evident that FADE effectively erases the target concept while preserving adjacent ones, outperforming the comparison algorithms by a significant margin across all three datasets, followed by SPM and CA. This demonstrates the superior capability at erasure and retention of the proposed FADE algorithm.

To evaluate FADE’s performance on adjacency retention, we analyze its classification accuracy across the top-10 adjacent classes for each target concept, as detailed in Table \ref{tab:similarity_scores}. This performance is measured using classifiers trained on the corresponding datasets. Figure \ref{fig:top-10} illustrates the retention accuracy for Stanford Dogs, Oxford Flowers, and CUB datasets. The results reveal a clear trend: as the similarity between concepts decreases (i.e., moving from the closest adjacent concept, A1, to the furthest, A10), retention performance improves. Notably, retention accuracy consistently remains above 75\%, showcasing FADE’s strong generalization capability on adjacent concepts even after the erasure of the target concept.


\begin{figure}[t]
\centering
  \includegraphics[width=0.5\textwidth]{Images/supp/Performance of FADE on top-10 Adjacency Classes.pdf}
\caption{For each target class in Table \ref{tab:similarity_scores}, we illustrate the performance of FADE on the top-10 adjacent classes. Adjacent classes are ordered by similarity scores. It is observed that FADE generalizes well on all adjacent classes after unlearning the target class.} 
    \label{fig:top-10}
\end{figure}



% To-Do's
% \textbf{Results of Table 1 on Top-10 classes. Detailed results of Table 2.}
% \textbf{Add reason behind choosing these concepts specifically.}
% Implementation Details.


\section{Extended Qualitative Results}
To provide a focused and detailed view of the results, Figures \ref{fig:FG_qualitative} and \ref{fig:CG_Qualitative} (borrowed from the main paper) visualize the performance of various unlearning algorithms.

Figure \ref{fig:FG_qualitative}, \ref{fig:dogs_quali}, \ref{fig:flowers_quali}, and \ref{fig:birds_quali} present the generation results for one target class and its adjacency set from each dataset, before and after applying unlearning algorithms. The first row in each of these figures displays images generated by the original Stable Diffusion (SD) model, followed by outputs from each unlearning method. Consistent with the quantitative results in Table 1 (main paper), ESD, FMN, and Receler fail to retain fine-grained details of neighboring classes. CA and SPM perform slightly better, retaining general structural features, but they struggle with specific attributes such as color and texture, especially in examples like dog breeds (e.g., Brittany Spaniel, Cocker Spaniel), bird species (e.g., Florida Jay, Cardinal), and flower species. These methods often result in incomplete erasure of the target concept or generalized representations of neighboring classes.

In contrast, FADE achieves a superior balance by effectively erasing the target concept while preserving the fine-grained details of related classes, as demonstrated by the sharper distinctions in the adjacency sets. FADE’s capability is further evaluated on ImageNet-1k for target classes such as Balls, Trucks, Dogs, and Fish. Table \ref{tab:similarity_scores} lists the neghiboring classes identified using Concept Lattice to construct the adjacency set for each target class. Notably, adjacency sets generated by Concept Lattice closely align with the manually curated fine-grained class structures reported by Peychev et al. \cite{peychev2023automated}, validating the accuracy and reliability of Concept Lattice.

As shown in Table 2 of the main paper, FADE outperforms all baseline methods, achieving at least a 12\% higher ERB score compared to SPM, the next-best algorithm. FMN and CA exhibit poor performance in both adjacency retention and erasure tasks, highlighting the robustness of FADE in fine-grained unlearning scenarios.


Further, human evaluation results for FADE and baseline algorithms are presented in Table \ref{tab:user_study}, capturing erasing accuracy ($A_{\text{er}}$) and average adjacency retention accuracy ($\hat{A}_{\text{adj}}$). We also capture their balance through the proposed Erasing-Retention Balance (ERB) score.

According to human evaluators, Receler achieves the highest $A_{\text{er}}$ (86.66\%) but fails in adjacency retention, with $\hat{A}{\text{adj}}$ close to zero, resulting in a minimal ERB score (0.06). FMN and CA show suboptimal performance, with FMN favoring erasure and CA favoring retention, yielding ERB scores of 43.07 and 38.43, respectively.

FADE outperforms all baselines with the highest ERB score (59.49), balancing effective erasure ($A_{\text{er}}$ of 51.94\%) and strong adjacency retention ($\hat{A}_{\text{adj}}$ of 69.62\%). These results highlight FADE’s ability to achieve adjacency-aware unlearning without significant collateral forgetting, setting a benchmark for fine-grained erasure tasks.

\begin{table}[t]
\centering
\begin{tabular}{lccc}
\hline
            & $A_{\text{er}}$        & $\hat{A}_{\text{adj}}$      & ERB   \\ \hline
ESD         & 73.33          & 37.22          & 49.38 \\
FMN         & 49.16          & 38.33          & 43.07 \\
CA          & 30.13          & 53.05          & 38.43 \\
SPM         & 40.83          & 61.66 & 49.13 \\
Receler     & \textbf{86.66} & 0.03           & 0.06  \\
FADE (ours) & 51.94          & \textbf{69.62}         & \textbf{59.49} \\ \hline
\end{tabular}
\caption{\label{tab:user_study}\textbf{Comparison of FADE with state-of-the-art unlearning methods based on evaluations by human participants.} If prediction of human evaluator is correct, a score of 1 was given; otherwise, a score of 0 was given. The performance is reported as a percentage. According to the user study, FADE effectively balances the erasure of the target concept with the retention of neighboring concepts.}
\end{table}

\section{Concept Unlearning Induces Concept Redirection}
Our experiments reveal an intriguing phenomenon where unlearning a target concept often results in its redirection to an unrelated concept. As illustrated in Figure \ref{fig:redirection}, this effect is particularly evident with algorithms like ESD and Receler. For example, after unlearning the “Blanket Flower,” the model generates a “girl with a black eye” when prompted for “Black-eyed Susan flower” and produces an image of “a man named William” for the prompt “Sweet William flower.” Similarly, for bird classes such as “Cliff Swallow” and “Tree Swallow,” the unlearning process redirects the concepts to unrelated outputs, such as trees or cliffs.

Interestingly, this redirection is primarily observed in algorithms like ESD and Receler, which struggle to maintain semantic coherence post-unlearning. In contrast, SPM and the proposed FADE algorithm demonstrate robust performance, effectively erasing the target concept without inducing unintended redirections, thereby preserving the model’s semantic integrity.






% Table for Fine-Grained Unlearning on Stanford Dogs dataset
\begin{table*}[t]
\centering
\footnotesize
\begin{tabular}{llccccccc}
\hline
                                                        &                                             & SD (Original) & ESD & FMN  & CA   & SPM  & Receler & FADE (ours) \\ \hline
\multicolumn{1}{l|}{Target Concept - 1}                 & \multicolumn{1}{l|}{Welsh Springer Spaniel} & 99.10          & 0.00   & 1.24  & 37.00   & 42.27 & 0.00       & 0.45         \\ \hline
\multicolumn{1}{l|}{\multirow{5}{*}{Adjacent Concepts}} & \multicolumn{1}{l|}{Brittany Spaniel}       & 95.42          & 0.00   & 0.00    & 58.00   & 54.60 & 0.00       & 81.85        \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{English Springer}       & 89.72          & 0.00   & 0.00    & 51.00   & 24.40 & 0.00       & 89.86        \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{English Setter}         & 94.00            & 0.00   & 0.00    & 56.84 & 73.85 & 0.00       & 93.00          \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Cocker Spaniel}         & 98.85         & 40.00  & 0.00    & 82.25 & 84.10 & 0.00       & 98.82        \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Sussex Spaniel}         & 99.68          & 60.62  & 0.00    & 85.00   & 88.75 & 12.00      & 99.65        \\ \hline
                                                        &                                             &               &     &      &      &      &         &             \\ \hline
\multicolumn{1}{l|}{Target Concept - 2}                 & \multicolumn{1}{l|}{German Shepherd}        & 99.62          & 0.00   & 0.00    & 20.85 & 0.89  & 0.00      & 0.00           \\ \hline
\multicolumn{1}{l|}{\multirow{5}{*}{Adjacent Concepts}} & \multicolumn{1}{l|}{Malinois}               & 99.00            & 0.00   & 0.00    & 51.86 & 57.43 & 0.00       & 96.29        \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Rottweiler}             & 98.10          & 0.00   & 0.25  & 54.58 & 70.24 & 0.00       & 94.25        \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Norwegian elkhound}     & 99.76          & 10.00  & 0.00    & 63.00   & 59.00   & 0.00       & 99.65        \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Labrador retriever}     & 95.00            & 30.00  & 1.86  & 73.60 & 73.65 & 0.00       & 88.20        \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Golden retriever}       & 99.86          & 60.00  & 0.88 & 75.44 & 93.81 & 14.00      & 99.44        \\ \hline
                                                        &                                             &               &     &      &      &      &         &             \\ \hline
\multicolumn{1}{l|}{Target Concept - 3}                 & \multicolumn{1}{l|}{Pomeranian}             & 99.84          & 0.00   & 1.85  & 32.00   & 66.49 & 0.00       & 0.24        \\ \hline
\multicolumn{1}{l|}{\multirow{5}{*}{Adjacent Concepts}} & \multicolumn{1}{l|}{Pekinese}               & 98.27          & 0.00   & 0.00    & 64.63 & 86.29 & 0.00       & 84.24       \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Yorkshire Terrier}      & 99.90          & 40.00  & 0.00    & 89.00   & 98.62 & 0.64     & 99.62        \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Shih Tzu}               & 98.85          & 60.00  & 0.00    & 92.00   & 95.65 & 2.55       & 93.65        \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Chow}                   & 100.00           & 10.00  & 1.20  & 87.60 & 98.22 & 3.27     & 100.00         \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Maltese dog}            & 99.45          & 60.00  & 1.86  & 88.88 & 97.45 & 0.00       & 96.45        \\ \hline
\end{tabular}
\caption{\label{tab:adj_acc_stanford_dogs}\textbf{Comparison of Classification Accuracy on Stanford Dogs Dataset}. We compare the classification accuracy (in \%) of various models on classes from the Stanford Dogs dataset before and after unlearning on each class in the adjacency set. The original model (SD) has not undergone any unlearning (higher accuracy is better), while the rest are comparison unlearning algorithms. For each algorithm, the model should exhibit lower accuracy on the target class and higher accuracy on the adjacent concepts. It is evident that FADE significantly outperforms all the comparison algorithms.}
\end{table*}



% Table for Fine-Grained Unlearning on Oxford Flowers dataset
\begin{table*}[t]
\centering
\footnotesize
\begin{tabular}{llccccccc}
\hline
                                                        &                                        & SD (Original) & ESD & FMN  & CA    & SPM  & Receler & Ours \\ \hline
\multicolumn{1}{l|}{Target Concept}                     & \multicolumn{1}{l|}{Barbeton Daisy}    & 91.50          & 0.00   & 24.45 & 29.89  & 30.00   & 0.00       & 0.12 \\ \hline
\multicolumn{1}{l|}{\multirow{5}{*}{Adjacent Concepts}} & \multicolumn{1}{l|}{Oxeye-Daisy}       & 99.15          & 20.00  & 4.20  & 75.60  & 86.86 & 1.85     & 95.24 \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Black Eyed Susan}  & 97.77          & 70.00  & 2.20  & 79.08 & 94.00   & 6.00       & 94.25 \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Osteospermum}      & 99.50          & 50.00  & 0.85  & 90.20  & 94.80 & 0.60    & 95.65 \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Gazania}           & 93.50          & 0.00   & 1.00    & 62.28  & 83.84 & 0.00       & 77.45 \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Purple Coneflower} & 99.80          & 100.00 & 1.65  & 85.80  & 98.85 & 23.22    & 99.87 \\ \hline
                                                        &                                        &               &     &      &       &      &         &      \\ \hline
\multicolumn{1}{l|}{Target Concept}                     & \multicolumn{1}{l|}{Yellow Iris}       & 99.30          & 0.00   & 0.00    & 32.45  & 51.69 & 0.00       & 0.00    \\ \hline
\multicolumn{1}{l|}{\multirow{5}{*}{Adjacent Concepts}} & \multicolumn{1}{l|}{Bearded Iris}      & 85.25          & 0.00   & 0.00    & 20.27  & 63.60 & 0.65     & 78.68 \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Canna Lily}        & 98.72          & 0.00   & 0.00    & 54.45  & 76.48 & 1.63    & 95.68 \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Daffodil}          & 94.65          & 10.00  & 5.25  & 59.89  & 88.00   & 0.00       & 92.45 \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Peruvian Lily}     & 98.50          & 20.00  & 0.00    & 64.00    & 88.20 & 0.00       & 93.45 \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Buttercup}         & 98.00            & 0.00   & 32.00   & 78.46  & 92.23 & 0.48     & 94.00   \\ \hline
                                                        &                                        &               &     &      &       &      &         &      \\ \hline
\multicolumn{1}{l|}{Target Concept}                     & \multicolumn{1}{l|}{Blanket Flower}    & 99.50          & 0.00   & 37.00   & 73.00    & 46.00   & 0.00       & 0.00    \\ \hline
\multicolumn{1}{l|}{\multirow{5}{*}{Adjacent Concepts}} & \multicolumn{1}{l|}{English Marigold}  & 99.56          & 0.00   & 3.00    & 94.25  & 98.00   & 0.00      & 99.43 \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Gazania}           & 93.55          & 0.00   & 0.00    & 66.87  & 74.24 & 0.00       & 83.00   \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Black Eyed Susan}  & 97.77          & 0.00   & 0.47  & 72.84  & 93.45 & 1.27     & 97.00   \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Sweet William}     & 97.75          & 0.00   & 0.68  & 66.62  & 70.00   & 2.45     & 93.88 \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Osteospermum}      & 99.50          & 20.00  & 0.25  & 92.68  & 86.45 & 0.83     & 83.20 \\ \hline
\end{tabular}
\caption{\label{tab:adj_acc_oxford_flowers}\textbf{Comparison of Classification Accuracy on Oxford Flower Dataset}. We compare the classification accuracy (in \%) of various models on classes from the Oxford Flower dataset before and after unlearning on each class in the adjacency set. The original model (SD) has not undergone any unlearning (higher accuracy is better), while the rest are comparison unlearning algorithms. For each algorithm, the model should exhibit lower accuracy on the target class and higher accuracy on the adjacent concepts. It is evident that FADE significantly outperforms all the comparison algorithms.}
\end{table*}



% Table for Fine-Grained Unlearning on CUB dataset

\begin{table*}[t]
\centering
\footnotesize
\begin{tabular}{llccccccc}
\hline
                                                        &                                              & SD (Original) & ESD      & FMN  & CA   & SPM  & Receler & Ours \\ \hline
\multicolumn{1}{l|}{Target Concept}                     & \multicolumn{1}{l|}{Blue Jay}                & 99.85          & 0.00        & 0.00    & 31.42 & 14.68 & 0.00       & 0.00   \\ \hline
\multicolumn{1}{l|}{\multirow{5}{*}{Adjacent Concepts}} & \multicolumn{1}{l|}{Florida Jay}             & 98.55          & 0.00        & 1.40  & 46.25 & 69.88 & 0.00       & 98.24 \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{White Breasted Nuthatch} & 99.00            & 5.00 & 0.00    & 72.00   & 85.08 & 0.00       & 98.44 \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Green Jay}               & 99.90          & 10.00       & 0.26  & 52.00   & 85.00   & 0.00       & 99.20 \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Cardinal}                & 100.00           & 30.00      & 0.11 & 86.85 & 96.43 & 3.48     & 100.00  \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Blue Winged Warbler}     & 92.97          & 20.00       & 0.54  & 49.28 & 64.24 & 0.00       & 90.65 \\ \hline
                                                        &                                              &               &          &      &      &      &         &      \\ \hline
\multicolumn{1}{l|}{Target Concept}                     & \multicolumn{1}{l|}{Black Tern}              & 86.65          & 0.00        & 4.00    & 22.45 & 13.87 & 0.00       & 0.00    \\ \hline
\multicolumn{1}{l|}{\multirow{5}{*}{Adjacent Concepts}} & \multicolumn{1}{l|}{Forsters Tern}           & 92.35          & 0.00        & 2.86  & 35.29 & 41.20 & 0.00       & 90.65 \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Long Tailed Jaeger}      & 97.66          & 30.00       & 9.85  & 81.08 & 90.67 & 0.66     & 90.84 \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Artic Tern}              & 89.50          & 0.00        & 0.45  & 22.20 & 37.85 & 0.00       & 90.26 \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Pomarine Jaeger}         & 88.29          & 0.00        & 0.82  & 52.80 & 63.64 & 0.00       & 80.85 \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Common Tern}             & 98.10          & 10.00       & 0.60  & 78.20 & 77.46 & 0.00       & 96.45 \\ \hline
                                                        &                                              &               &          &      &      &      &         &      \\ \hline
\multicolumn{1}{l|}{Target Concept}                     & \multicolumn{1}{l|}{Barn Swallow}            & 99.40          & 0.00        & 1.25  & 57.06 & 7.48  & 0.00       & 0.45  \\ \hline
\multicolumn{1}{l|}{\multirow{5}{*}{Adjacent Concepts}} & \multicolumn{1}{l|}{Bank Swallow}            & 9.79           & 0.00        & 0.65  & 54.60 & 30.21 & 0.00       & 93.60 \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Lazuli Bunting}          & 99.75          & 70.00       & 0.65  & 82.00   & 88.40 & 0.00       & 99.00   \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Cliff Swallow}           & 93.20          & 0.00        & 0.00    & 77.00   & 47.63 & 0.86     & 91.25 \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Indigo Bunting}          & 96.80          & 70.00       & 17.46 & 87.68 & 93.00   & 5.22     & 96.45 \\
\multicolumn{1}{l|}{}                                   & \multicolumn{1}{l|}{Cerulean Warbler}        & 96.90          & 50.00       & 2.65  & 88.40 & 89.00   & 0.45     & 96.80 \\ \hline
\end{tabular}
\caption{\label{tab:adj_acc_cub}\textbf{Comparison of Classification Accuracy on CUB Dataset}. We compare the classification accuracy (in \%) of various models on classes from the CUB dataset before and after unlearning on each class in the adjacency set. The original model (SD) has not undergone any unlearning (higher accuracy is better), while the rest are comparison unlearning algorithms. For each algorithm, the model should exhibit lower accuracy on the target class and higher accuracy on the adjacent concepts. It is evident that FADE significantly outperforms all the comparison algorithms.}
\end{table*}


% Table of Adjacency Set with their similarity scores.
\begin{sidewaystable*}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc}
\hline
\multicolumn{1}{l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Stanford Dogs\\ Dataset\end{tabular}}} & \multicolumn{2}{c|}{Welsh Springer Spaniel}                         & \multicolumn{2}{c|}{German Shepherd}                              & \multicolumn{2}{c}{Pomeranian}                 \\
\multicolumn{1}{l|}{}                                                                                 & Class Names                 & \multicolumn{1}{c|}{Similarity Score} & Class Names               & \multicolumn{1}{c|}{Similarity Score} & Class Names                 & Similarity Score \\ \hline
\multicolumn{1}{l|}{Adjacent Class - 1}                                                               & Brittany Spaniel            & \multicolumn{1}{c|}{98.19}            & Malinois                  & \multicolumn{1}{c|}{95.84}            & Pekinese                    & 92.67            \\
\multicolumn{1}{l|}{Adjacent Class - 2}                                                               & English Springer            & \multicolumn{1}{c|}{97.05}            & Rottweiler                & \multicolumn{1}{c|}{92.52}            & Yorkshire Terrier           & 92.42            \\
\multicolumn{1}{l|}{Adjacent Class - 3}                                                               & English Setter              & \multicolumn{1}{c|}{95.12}            & Norwegian Walkhound       & \multicolumn{1}{c|}{92.51}            & Shih Tzu                    & 91.58            \\
\multicolumn{1}{l|}{Adjacent Class - 4}                                                               & Cocker Spaniel              & \multicolumn{1}{c|}{95.10}            & Labrador Retriever        & \multicolumn{1}{c|}{91.63}            & Chow                        & 90.99            \\
\multicolumn{1}{l|}{Adjacent Class - 5}                                                               & Sussex Spaniel              & \multicolumn{1}{c|}{93.62}            & Golden Retriever          & \multicolumn{1}{c|}{91.43}            & Maltese Dog                 & 90.96            \\
\multicolumn{1}{l|}{Adjacent Class - 6}                                                               & Blenheim Spaniel            & \multicolumn{1}{c|}{93.05}            & Collie                    & \multicolumn{1}{c|}{90.79}            & Chihuaha                    & 90.49            \\
\multicolumn{1}{l|}{Adjacent Class - 7}                                                               & Irish Setter                & \multicolumn{1}{c|}{92.90}            & Doberman                  & \multicolumn{1}{c|}{90.37}            & Papillon                    & 90.38            \\
\multicolumn{1}{l|}{Adjacent Class - 8}                                                               & Saluki                      & \multicolumn{1}{c|}{92.83}            & Black and Tan Coonhound   & \multicolumn{1}{c|}{90.27}            & Samoyed                     & 89.22            \\
\multicolumn{1}{l|}{Adjacent Class - 9}                                                               & English Foxhound            & \multicolumn{1}{c|}{92.81}            & Bernese Mountain dog      & \multicolumn{1}{c|}{90.06}            & Australian Terrier          & 89.15            \\
\multicolumn{1}{l|}{Adjacent Class - 10}                                                              & Gordon Setter               & \multicolumn{1}{c|}{92.35}            & Border collie             & \multicolumn{1}{c|}{89.56}            & Toy poodle                  & 89.05            \\ \hline
                                                                                                      &                             &                                       &                           &                                       &                             &                  \\ \hline
\multicolumn{1}{l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Oxford Flower\\ Dataset\end{tabular}}} & \multicolumn{2}{c|}{Barbeton Daisy}                                 & \multicolumn{2}{c|}{Yellow Iris}                                  & \multicolumn{2}{c}{Blanket Flower}             \\
\multicolumn{1}{l|}{}                                                                                 & Class Names                 & \multicolumn{1}{c|}{Similarity Score} & Class Names               & \multicolumn{1}{c|}{Similarity Score} & Class Names                 & Similarity Score \\ \hline
\multicolumn{1}{l|}{Adjacent Class - 1}                                                               & Oxeye Daisy                 & \multicolumn{1}{c|}{98.65}            & Bearded Iris              & \multicolumn{1}{c|}{96.38}            & English Marigold            & 95.13            \\
\multicolumn{1}{l|}{Adjacent Class - 2}                                                               & Black eyed susan            & \multicolumn{1}{c|}{95.56}            & Canna Lily                & \multicolumn{1}{c|}{92.48}            & Gazania                     & 92.38            \\
\multicolumn{1}{l|}{Adjacent Class - 3}                                                               & Osteospermum                & \multicolumn{1}{c|}{94.99}            & Daffodil                  & \multicolumn{1}{c|}{92.33}            & Black Eyed Susan            & 90.64            \\
\multicolumn{1}{l|}{Adjacent Class - 4}                                                               & Gazania                     & \multicolumn{1}{c|}{93.91}            & Peruvian Lily             & \multicolumn{1}{c|}{92.18}            & Sweet William               & 90.00            \\
\multicolumn{1}{l|}{Adjacent Class - 5}                                                               & Purple Coneflower           & \multicolumn{1}{c|}{93.27}            & Buttercup                 & \multicolumn{1}{c|}{91.55}            & Osteospermum                & 89.94            \\
\multicolumn{1}{l|}{Adjacent Class - 6}                                                               & Pink yellow dahlia          & \multicolumn{1}{c|}{91.74}            & Hippeastrum               & \multicolumn{1}{c|}{91.33}            & Barbeton Daisy              & 89.86            \\
\multicolumn{1}{l|}{Adjacent Class - 7}                                                               & Sunflower                   & \multicolumn{1}{c|}{91.18}            & Moon Orchid               & \multicolumn{1}{c|}{91.08}            & Purple Coneflower           & 89.45            \\
\multicolumn{1}{l|}{Adjacent Class - 8}                                                               & Buttercup                   & \multicolumn{1}{c|}{91.17}            & Ruby Lipped Cattleya      & \multicolumn{1}{c|}{90.75}            & Snapdragon                  & 89.42            \\
\multicolumn{1}{l|}{Adjacent Class - 9}                                                               & Japanese Anemone            & \multicolumn{1}{c|}{90.56}            & Hard-Leaved Pocket Orchid & \multicolumn{1}{c|}{90.36}            & Wild Pansy                  & 88.06            \\
\multicolumn{1}{l|}{Adjacent Class - 10}                                                              & Magnolia                    & \multicolumn{1}{c|}{90.27}            & Azalea                    & \multicolumn{1}{c|}{90.02}            & Pink Yellow Dahlia          & 88.01            \\ \hline
                                                                                                      &                             &                                       &                           &                                       &                             &                  \\ \hline
\multicolumn{1}{l|}{\multirow{2}{*}{CUB Dataset}}                                                     & \multicolumn{2}{c|}{Blue Jay}                                       & \multicolumn{2}{c|}{Black Tern}                                   & \multicolumn{2}{c}{Barn Swallow}               \\
\multicolumn{1}{l|}{}                                                                                 & Class Names                 & \multicolumn{1}{c|}{Similarity Score} & Class Names               & \multicolumn{1}{c|}{Similarity Score} & Class Names                 & Similarity Score \\ \hline
\multicolumn{1}{l|}{Adjacent Class - 1}                                                               & Florida Jay                 & \multicolumn{1}{c|}{93.62}            & Forsters Tern             & \multicolumn{1}{c|}{96.19}            & Bank Swallow                & 95.91            \\
\multicolumn{1}{l|}{Adjacent Class - 2}                                                               & White Breasted Nuthatch     & \multicolumn{1}{c|}{92.50}            & Long Tailed Jaeger        & \multicolumn{1}{c|}{95.54}            & Lazuli Bunting              & 93.91            \\
\multicolumn{1}{l|}{Adjacent Class - 3}                                                               & Green Jay                   & \multicolumn{1}{c|}{91.91}            & Artic Tern                & \multicolumn{1}{c|}{94.79}            & Cliff Swallow               & 92.47            \\
\multicolumn{1}{l|}{Adjacent Class - 4}                                                               & Cardinal                    & \multicolumn{1}{c|}{90.86}            & Pomarine Jaeger           & \multicolumn{1}{c|}{94.52}            & Indigo Bunting              & 92.04            \\
\multicolumn{1}{l|}{Adjacent Class - 5}                                                               & Blue Winged Warbler         & \multicolumn{1}{c|}{90.00}            & Common Tern               & \multicolumn{1}{c|}{93.35}            & Cerulean Warbler            & 91.65            \\
\multicolumn{1}{l|}{Adjacent Class - 6}                                                               & Downy Woodpecker            & \multicolumn{1}{c|}{88.84}            & Elegant Tern              & \multicolumn{1}{c|}{93.03}            & Blue Grosbeak               & 91.58            \\
\multicolumn{1}{l|}{Adjacent Class - 7}                                                               & Indigo Bunting              & \multicolumn{1}{c|}{88.83}            & Frigatebird               & \multicolumn{1}{c|}{91.32}            & Tree Swallow                & 91.33            \\
\multicolumn{1}{l|}{Adjacent Class - 8}                                                               & Cerulean Warbler            & \multicolumn{1}{c|}{88.80}            & Least tern                & \multicolumn{1}{c|}{91.28}            & Black Throated Blue Warbler & 90.43            \\
\multicolumn{1}{l|}{Adjacent Class - 9}                                                               & Black Throated Blue Warbler & \multicolumn{1}{c|}{88.64}            & Red legged Kittiwake      & \multicolumn{1}{c|}{91.22}            & Blue winged warbler         & 89.25            \\
\multicolumn{1}{l|}{Adjacent Class - 10}                                                              & Clark Nutcracker            & \multicolumn{1}{c|}{88.39}            & Lysan Albatross           & \multicolumn{1}{c|}{90.17}            & White breasted kingfisher   & 89.16            \\ \hline
\end{tabular}
}
\caption{\label{tab:similarity_scores}Description of the adjacency set for target classes from the Stanford Dogs, Oxford Flowers, and CUB datasets, along with their similarity scores.}
\end{sidewaystable*}



% \begin{sidewaysfigure}
\begin{figure*}
\centering
% \includegraphics[width=\textheight]{Images/FADE_qualitative_results_1.pdf}
\includegraphics[width=\textwidth]{Images/FADE_qualitative_results_1.pdf}
\caption{\textbf{Qualitative comparison between existing and proposed algorithms for erasing target concepts and testing retention on neighboring fine-grained concepts.} Results are shown for one target concept each from the Stanford Dogs, Oxford Flowers, and CUB datasets.}
\label{fig:FG_qualitative}
\end{figure*}
% \end{sidewaysfigure}




\begin{figure*}[t]
\centering
  \includegraphics[width=\textwidth]{Images/FADE_qualitative_results_1_I10.pdf}
\caption{Comparison of FADE with various algorithms for erasing the 'garbage truck' class in Fine-Grained and Coarse-Grained Unlearning. The target class, adjacency set and the retain set and constructed from the ImageNet-1k dataset.} 
    \label{fig:CG_Qualitative}
\end{figure*}

\begin{figure*}[t]
\centering
  \includegraphics[width=\textwidth]{Images/supp/_FADE_qualitative_dogs_suppl.pdf}
\caption{Qualitative comparison of FADE with various algorithms for erasing German Shepherd and Pomeranian while retaining closely looking breeds extracted through concept lattice from the Stanford Dogs dataset.} 
    \label{fig:dogs_quali}
\end{figure*}

\begin{figure*}[t]
\centering
  \includegraphics[width=\textwidth]{Images/supp/_FADE_qualitative_flowers_suppl.pdf}
\caption{Qualitative comparison of FADE with various algorithms for erasing Yellow Iris and Blanket Flower while retaining other similar-looking flowers through concept lattice from the Oxford Flowers dataset.} 
    \label{fig:flowers_quali}
\end{figure*}

\begin{figure*}[t]
\centering
  \includegraphics[width=\textwidth]{Images/supp/FADE_qualitative_birds_suppl.pdf}
\caption{Qualitative comparison of FADE with various algorithms for erasing Blank Tern and Barn Swallow while retaining other closely looking bird species extracted through concept lattice from CUB dataset.} 
    \label{fig:birds_quali}
\end{figure*}


\begin{figure*}[t]
\centering
  \includegraphics[width=\textwidth]{Images/supp/concept_redirection.pdf}
\caption{  \label{fig:redirection}Illustration of concept redirection observed after unlearning target concepts using various algorithms. For ESD and Receler, the erasure of “Blanket Flower” redirects to unrelated outputs, such as a “girl with a black eye” for “Black-eyed Susan flower” and “a man named William” for “Sweet William flower.” Similar redirection is seen with bird classes like “Cliff Swallow” and “Tree Swallow.” In contrast, SPM and FADE effectively erase target concepts without inducing semantic redirection, ensuring coherence and retention of related knowledge.} 
  
\end{figure*}


% \begin{figure*}[t]
% \centering
%   \includegraphics[width=\textwidth]{Images/supp/FADE_qualitative_results_1_break_1.pdf}
% \caption{Comparison of FADE with various algorithms for erasing the 'garbage truck' class in Fine-Grained and Coarse-Grained Unlearning. The target class, adjacency set and the retain set and constructed from the ImageNet-1k dataset.} 
%     \label{fig:CG_Qualitative}
% \end{figure*}

% \begin{figure}[t]
% \centering
%   \includegraphics[width=\textwidth]{Images/supp/FADE_qualitative_results_1_break_2.pdf}
% \caption{Comparison of FADE with various algorithms for erasing the 'garbage truck' class in Fine-Grained and Coarse-Grained Unlearning. The target class, adjacency set and the retain set and constructed from the ImageNet-1k dataset.} 
%     \label{fig:CG_Qualitative}
% \end{figure}







% \section{Concept Unlearning leads to Concept Redirection}
% \textbf{Another figure on unleaning Analysis.} The Cliff wala example.


% % 

% Having the supplementary compiled together with the main paper means that:
% % 
% \begin{itemize}
% \item The supplementary can back-reference sections of the main paper, for example, we can refer to \cref{sec:intro};
% \item The main paper can forward reference sub-sections within the supplementary explicitly (e.g. referring to a particular experiment); 
% \item When submitted to arXiv, the supplementary will already included at the end of the paper.
% \end{itemize}
% % 
% To split the supplementary pages from the main paper, you can use \href{https://support.apple.com/en-ca/guide/preview/prvw11793/mac#:~:text=Delete%20a%20page%20from%20a,or%20choose%20Edit%20%3E%20Delete).}{Preview (on macOS)}, \href{https://www.adobe.com/acrobat/how-to/delete-pages-from-pdf.html#:~:text=Choose%20%E2%80%9CTools%E2%80%9D%20%3E%20%E2%80%9COrganize,or%20pages%20from%20the%20file.}{Adobe Acrobat} (on all OSs), as well as \href{https://superuser.com/questions/517986/is-it-possible-to-delete-some-pages-of-a-pdf-document}{command line tools}.
